Rationalizability and Epistemic Priority Orderings

At the beginning of a dynamic game, players may have exogenous theories about how the opponents are going to play. Suppose that these theories are commonly known. Then, players will refine their first-order beliefs, and challenge their own theories, through strategic reasoning. I develop and characterize epistemically a new solution concept, Selective Rationalizability, which accomplishes this task under the following assumption: when the observed behavior is not compatible with the beliefs in players' rationality and theories of all orders, players keep the orders of belief in rationality that are per se compatible with the observed behavior, and drop the incompatible beliefs in the theories. Thus, Selective Rationalizability captures Common Strong Belief in Rationality (Battigalli and Siniscalchi, 2002) and refines Extensive-Form Rationalizability (Pearce, 1984; BS, 2002), whereas Strong-$\Delta$-Rationalizability (Battigalli, 2003; Battigalli and Siniscalchi, 2003) captures the opposite epistemic priority choice. Selective Rationalizability can be extended to encompass richer epistemic priority orderings among different theories of opponents' behavior. This allows to establish a surprising connection with strategic stability (Kohlberg and Mertens, 1986).

==> eptcsdata.tex <==
\providecommand{\firstpage}{102}
\providecommand{\publicationstatus}{J. Lang (Ed.): TARK 2017\\
EPTCS 251, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.251.8}{10.4204/EPTCS.251.8}}

